Search For Higgs Boson Pair Production in the $\gamma\gamma b\bar{b}$ Final State using $pp$ Collision Data at $\sqrt{s}=8$ TeV from the ATLAS Detector

Searches are performed for resonant and non-resonant Higgs boson pair production in the $\gamma\gamma b\bar{b}$ final state using 20 fb$^{-1}$ of proton-proton collisions at a center-of-mass energy of 8 TeV recorded with the ATLAS detector at the CERN Large Hadron Collider. A 95% confidence level upper limit on the cross section times branching ratio of non-resonant production is set at 2.2 pb, while the expected limit is 1.0 pb. The difference derives from a modest excess of events, corresponding to 2.4 standard deviations from the background-only hypothesis. The limit observed in the search for a narrow $X \to hh$ resonance ranges between 0.7 and 3.5 pb as a function of the resonance mass.

==> title_and_abstract.tex <==
Search for Higgs Boson Pair Production in the $\gamma\gamma b\bar{b}$ Final State using $pp$ Collision Data at $\sqrt{s}=8$~TeV from the ATLAS Detector

Searches are performed for resonant and non-resonant Higgs boson pair production in the $hh \rightarrow \gamma\gamma b \overline b$ final state using 20 fb$^{-1}$ of proton--proton collisions at a center-of-mass energy of 8~TeV recorded with the ATLAS detector at the CERN Large Hadron Collider. A 95\% confidence level upper limit on the cross section times branching ratio of non-resonant production is set at 2.2~pb, while the expected limit is 1.0~pb. The corresponding limit observed for a narrow resonance ranges between 0.7 and 3.5~pb as a function of its mass.

